On the Potential of Simple Framewise Approaches to Piano Transcription

In an attempt at exploring the limitations of simple approaches to the task of piano transcription (as usually defined in MIR), we conduct an in-depth analysis of neural network-based framewise transcription. We systematically compare different popular input representations for transcription systems to determine the ones most suitable for use with neural networks. Exploiting recent advances in training techniques and new regularizers, and taking into account hyper-parameter tuning, we show that it is possible, by simple bottom-up frame-wise processing, to obtain a piano transcriber that outperforms the current published state of the art on the publicly available MAPS dataset -- without any complex post-processing steps. Thus, we propose this simple approach as a new baseline for this dataset, for future transcription research to build on and improve.

==> figs/definitive/cleaned_all/table.tex <==
Learning Rate (21.1\%) & Learning Rate $\times$ Model Class (10.0\%) & Model Class $\times$ Spectrogram Type (9.4\%) & Spectrogram Type (9.4\%) & Model Class (6.1\%) & Learning Rate $\times$ Spectrogram Type (4.1\%) & Spectrogram Type $\times$ Sample Rate (2.2\%) & $L_2$ Penalty (2.0\%) & Dropout $\times$ Spectrogram Type (1.9\%) & Dropout (1.7\%) & 

==> figs/definitive/cleaned_all_shallow/table.tex <==
Learning Rate (47.7\%) & Spectrogram Type (13.0\%) & Learning Rate $\times$ Spectrogram Type (6.1\%) & Dropout (4.1\%) & Dropout $\times$ Spectrogram Type (3.9\%) & Optimizer $\times$ Spectrogram Type (2.3\%) & Optimizer (2.2\%) & Learning Rate $\times$ Dropout (1.8\%) & Spectrogram Type $\times$ Sample Rate (1.6\%) & Learning Rate $\times$ Optimizer (1.1\%) & 

==> figs/definitive/cleaned_final_shallow/table.tex <==
Learning Rate (33.4\%) & Dropout (8.5\%) & Learning Rate $\times$ Dropout (6.8\%) & Dropout $\times$ Spectrogram Type (6.2\%) & Spectrogram Type (5.5\%) & Batch Normalization (5.0\%) & Dropout $\times$ Batch Normalization (3.9\%) & Learning Rate $\times$ Spectrogram Type (3.5\%) & Optimizer (1.8\%) & Batch Normalization $\times$ Spectrogram Type (1.5\%) & 

==> figs/definitive/cleaned_latest_shallow/table.tex <==
Learning Rate (47.1\%) & Spectrogram Type (5.3\%) & Dropout (4.4\%) & Optimizer (3.9\%) & Batch Normalization (3.6\%) & Dropout $\times$ Spectrogram Type (3.6\%) & Learning Rate $\times$ Spectrogram Type (3.4\%) & Optimizer $\times$ Spectrogram Type (3.2\%) & Learning Rate $\times$ Dropout (2.6\%) & Learning Rate $\times$ Optimizer (1.4\%) & 

==> figs/definitive/cleaned_latest_shallow_logscale/table.tex <==
Learning Rate (47.1\%) & Spectrogram Type (5.3\%) & Dropout (4.4\%) & Optimizer (3.9\%) & Batch Normalization (3.6\%) & Dropout $\times$ Spectrogram Type (3.6\%) & Learning Rate $\times$ Spectrogram Type (3.4\%) & Optimizer $\times$ Spectrogram Type (3.2\%) & Learning Rate $\times$ Dropout (2.6\%) & Learning Rate $\times$ Optimizer (1.4\%) & 

==> figs/isolated_input_logreg/table.tex <==
Spectrogram Type (48.6\%) & Spectrogram Type $\times$ Normed Area Filters (16.9\%) & Spectrogram Type $\times$ Sample Rate (10.4\%) & 

==> figs/isolated_input_shallow/table.tex <==
Spectrogram Type (68.4\%) & Spectrogram Type $\times$ Sample Rate (20.8\%) & Sample Rate (5.7\%) & 
